Development of Linear Battery Model for Path Planning with Mixed Integer Linear Programming: Simulated and Experimental Validation

Mixed Integer Linear Programs (MILPs) are often used in the path planning of both ground and aerial vehicles. Such a formulation of the path planning problem requires a linear objective function and constraints, limiting the fidelity of the the tracking of vehicle states. One such parameter is the state of charge of the battery used to power the vehicle. Accurate battery state estimation requires nonlinear differential equations to be solved. This state estimation is important in path planning to ensure flyable paths, however when using MILPs to formulate the path planning problem these nonlinear equations cannot be implemented. Poor accuracy in battery estimation during the path planning runs the risk of the planned path being feasible by the estimation model but in reality will deplete the battery to a critical level. To the end of higher accuracy battery estimation within a MILP, we present here a simple linear battery model which predicts the change in state-of-charge (SOC) of a battery given a power draw and duration. This model accounts for changes in battery voltage due to applied electrical load and changes in battery SOC. The battery model is presented and then tested against alternate battery models in numerical and in experimental tests. Further, the effect the proposed linear model has over a simpler SOC estimation on the time-to-solve a resource constrained shortest path problem is also evaluated, implemented in two different algorithms. It is seen that the linear model performs well in battery state estimation while remaining implementable in a Linear Program or MILP, with little affect on the time-to-solve.

==> OCV18650.tex <==
\begin{table}
\vspace{.18cm}
\centering
% \resizebox{0.5\textwidth}{
\begin{tabular}{|c|c|c|c|}
% \scriptsize
\hline
SOC (\%) & OCV (V) \\ \hline
100.0 & 4.1617  \\ \hline
95.03 & 4.0913  \\ \hline
90.07 & 4.0749  \\ \hline
85.1 & 4.0606  \\ \hline
80.13 & 4.0153  \\ \hline
75.17 & 3.9592  \\ \hline
70.2 & 3.9164  \\ \hline
65.24 & 3.8687  \\ \hline
60.27 & 3.8163  \\ \hline
55.3 & 3.7735  \\ \hline
50.34 & 3.7317  \\ \hline
45.37 & 3.6892  \\ \hline
40.4 & 3.6396  \\ \hline
35.43 & 3.5677  \\ \hline
30.46 & 3.5208  \\ \hline
25.5 & 3.4712  \\ \hline
20.53 & 3.386  \\ \hline
15.56 & 3.288  \\ \hline
10.59 & 3.2037  \\ \hline
5.63 & 3.0747  \\ \hline

\end{tabular}%}
\caption{Open Circuit Voltage Data - 18650 Li-Ion Battery}\label{table/18650OCV}
\end{table}

==> OCV_lipo.tex <==
\begin{table}
\vspace{.18cm}
\centering
% \resizebox{0.5\textwidth}{
\begin{tabular}{|c|c|c|c|}
% \scriptsize
\hline
SOC (\%) & OCV (V) \\ \hline
 100.0 & 16.7884  \\ \hline 
 96.68 & 16.6217  \\ \hline
 93.45 & 16.4868  \\ \hline
 90.46 & 16.3925  \\ \hline
 87.25 & 16.3341  \\ \hline
 84.11 & 16.2829  \\ \hline
 70.2 & 16.0399  \\ \hline
 56.77 & 15.6845  \\ \hline
 43.67 & 15.4958  \\ \hline
 30.75 & 15.2911  \\ \hline
 25.11 & 15.1267  \\ \hline
 19.58 & 14.9496  \\ \hline
 14.13 & 14.8004  \\ \hline

\end{tabular}%}
\caption{Open Circuit Voltage Data - 6S LiPo}\label{table/lipoOCV}
\end{table}
